A water-obstacle separation and refinement network for unmanned surface vehicles

Obstacle detection by semantic segmentation shows a great promise for autonomous navigation in unmanned surface vehicles (USV). However, existing methods suffer from poor estimation of the water edge in the presence of visual ambiguities, poor detection of small obstacles and high false-positive rate on water reflections and wakes. We propose a new deep encoder-decoder architecture, a water-obstacle separation and refinement network (WaSR), to address these issues. Detection and water edge accuracy are improved by a novel decoder that gradually fuses inertial information from IMU with the visual features from the encoder. In addition, a novel loss function is designed to increase the separation between water and obstacle features early on in the network. Subsequently, the capacity of the remaining layers in the decoder is better utilised, leading to a significant reduction in false positives and increased true positives. Experimental results show that WaSR outperforms the current state-of-the-art by a large margin, yielding a 14% increase in F-measure over the second-best method.

==> cutout.tex <==
-----------------------------------------------------------
%
%This section introduces datasets used for training and evaluation of our method. \Cref{fig:dataset_images} visualises example images from each selected dataset to emphasise the diversity of marine environment.
%
For training purposes, we have used MaSTr1325 dataset~\cite{bb_iros_2019} which was captured by a real USV over a span of 24 months in the gulf of Koper, Slovenia. %During the dataset acquisition period, the USV was equipped with an IMU sensor and \emph{Vrmagic VRmMFC} stereo camera system, which is comprised of two \emph{Vrmagic VRmS-14/C-COB} CCD sensors with \SI{0.3}{\meter} baseline, \emph{Thorlabs MVL4WA} lens with \SI{3.5}{\milli\meter} focal length, maximum aperture of $\mathrm{f}/1.4$, and a \SI{132.1}{\degree} FOV. 
The dataset consists of $1325$ representative, high-resolution ($1278 \times 958$ pixels) images of a marine environment (visualised in \cref{fig:dataset_images} top row), which are manually annotated by human annotators for three semantic components (sea, sky and environment). The edges of the semantically different components are labelled with the ``unknown'' category in order to address the annotation uncertainty and to ensure that these pixels are excluded from learning. All images from the dataset are additionally synchronised with measurements from on-board IMU sensor.

%
%The evaluation procedure was carried out on two separate datasets (SMD~\cite{smd_prasad2017video} and Modd2~\cite{bb_ras_2018}) to demonstrate the independence of the method from the environment in which the USV operates. The selected datasets for evaluation were captured with different cameras in two completely different harbours at the opposing sides of the world. 

%Sequences from SMD~\cite{smd_prasad2017video} were acquired in the harbour of Singapore, Malaysia with \textit{Canon 70D} camera equipped with \textit{Canon EF 70-300mm f/4-5.6 IS USM} lens. The dataset consists of 81 full-HD ($1920 \times 1080$ pixels) sequences, which can be subdivided into three categories --- RGB on-shore (40 sequences), RGB on-board (11 sequences) and near infra-red on-shore (30 sequences). Due to the nature of our experiment we have limited ourselves to the RGB on-board sequences. 

The evaluation procedure was carried out on a standard Modd2 dataset~\cite{bb_ras_2018}.
%Sequences in Modd2 were captured in the gulf of Koper, Slovenia with the acquisition system described in \cref{subsubsec:training_set}.
It consists of 28 sequences which are time-synchronised with measurements of the on-board IMU. The bad weather conditions present in the dataset, make it the most challenging USV obstacle detection dataset to date. Example images from the dataset are visualized in the bottom row of \cref{fig:dataset_images}, where different weather conditions can be observed. Obstacles and water-edge in the dataset are manually annotated with bounding boxes and a polygon respectively. Since MaSTr1325 contains undistorted and non-rectified images, we have decided to use undistorted and non-rectified images for evaluation as well. 

----------------------------
Water separation loss:

To further supervise and guide the training procedure towards efficient segmentation of small obstacles we propose applying a novel \textit{water-separation} loss function on early features of the encoder. Its general purpose is to enforce separation of pixels belonging to the water component from pixels belonging to the obstacles component. By fitting a Gaussian distribution on pixels belonging to the water component, we can calculate the spread of the water component. Similarly, we can calculate the spread of the obstacle component with respect to the mean value of the water component. The proposed water-separation loss function is thus defined as
%
\begin{align}
    \mathcal{L}_{\mathrm{water-separation}} = \frac{1}{n_c} \sum_j^{n_c}{ \frac{ \frac{1}{n^{w,j}} \sum_i{ ({y_i}^{w,j} - \mu^{w,j})^2} }{ \frac{1}{n^{o,j}} \sum_i{ ({y_i}^{o,j} - \mu^{w,j})^2} } },
\end{align}
%
where ${y_i}^{w,j}$ denotes $i$-th pixel at $j$-th feature channel that belongs to the water component, ${y_i}^{o,j}$ denotes $i$-th pixel at $j$-th feature channel that belongs to the obstacles component, $n^{w,j}$ and $n^{o,j}$ denote the number of pixels belonging to the water component on $j$-th feature channel and the number of pixels belonging to the obstacles component on $j$-th feature channel respectively, while $n_c$ denotes the number of feature channels and $\mu_{w,j}$ the mean value of pixels belonging to the water component at $j$-th feature channel. The proposed water-separation function can be optimised by minimising the spread of the water component while maximising the spread of the obstacles component.

%Increasing the amount of epoch leads to more specialised weights for the training data, which results in over-fitting. In order to handle the specifics seen in the training data, the weights will grow in size. Large weights make the network unstable, resulting in poor performance on new data. In practice, we prefer simpler models with smaller weights. To guide the network training towards smaller weights, we combine the focal loss function and water-separation loss function with L2 regularisation~\cite{krogh1992simple}. 
%To handle over-fitting and guide the network training towards smaller weights we use standard L2 regularisation~\cite{krogh1992simple}. The final loss functions is a weighted summation, defines as
To handle regularisation of the weights we use standard L2 regularisation~\cite{krogh1992simple}.




--------------------------------------------------------------------------
The proposed USVNet (\cref{fig:intro_image}) has a non-symmetric architecture consisting of a \textit{contracting path} (encoder) and an \textit{expansive path} (decoder). The encoder is used to produce down-sampled feature maps, while the decoder is used to up-sample the feature maps, merge the visual information with the IMU measurements and recover %a certain extent of 
spatial information. Layers from both paths on corresponding levels are connected via skip-connections to avoid the vanishing gradient problem. \\

\textbf{Contraction path} uses ResNet-101~\cite{he2016deep} model with atrous convolutions to extract deep features from the input image. The aforementioned model is composed of four convolutional blocks (denoted as \textit{res2, res3, res4} and \textit{res5}) which, combined with max-pooling layers, handle the resolution reduction of the input image. Each convolutional block incorporates residual connections to address the vanishing gradient problem~\cite{he2016deep}. The last two convolutional blocks adopt hybrid atrous convolutions~\cite{wang2018understanding} to further increase the receptive field. Larger receptive field enables the encoding of a higher level semantic context information. In our previous work~\cite{bb_iros_2019} we have experimentally proven the importance of the atrous convolutions in the encoder.


%\textbf{Expansive path} has two purposes --- (i) fuse visual and inertial information and (ii) gradually recover object details and spatial dimensions. The fusion of features from different sources (e.g. camera, IMU) and/or layer levels is achieved by Feature Fusion Module (FFM). To further refine the fused features we propose applying Attention Refinement Module (ARM)~\cite{yu2018bisenet} after each FFM. Gradual recovery of object details and spatial dimensions is accomplished by deploying an incomplete U-shape structure~\cite{ronneberger2015u}, connecting features from different levels of contraction path with features, enriched by the IMU information, on corresponding levels of the expensive path. The expansive path stops, when the feature map in the up-sampling process reaches half the size of the input image, forming the incomplete U-shape structure. Applying Atrous Spatial Pyramid Pooling (ASPP) module on halved resolution reduces the computational complexity, while simultaneously increasing the receptive field, leading to a better segmentation output.
\textbf{Expansive path} has two purposes --- (i) fuse visual with inertial information and (ii) gradually recover object details and spatial dimensions. The inertial information is introduced into the network at two different layer levels. The fusion of features from different sources (camera and IMU) is achieved by concatenation, followed by modified Attention Refinement Module (ARM)~\cite{yu2018bisenet}, which further refines the fused features. Gradual recovery of object details and spatial dimensions is accomplished by deploying an incomplete U-shape structure~\cite{ronneberger2015u}, connecting features from different levels of contraction path with features, enriched by the IMU information, on corresponding levels of the expensive path. To fuse features from different layer levels in the expensive path we propose using a modified Feature Fusion Module (FFM)~\cite{yu2018bisenet}. The expansive path stops, when the feature map in the up-sampling process reaches quarter the size of the input image, forming the incomplete U-shape structure. Applying Atrous Spatial Pyramid Pooling (ASPP) module on lower resolution reduces the computational complexity, while simultaneously increasing the receptive field, leading to a better segmentation output. The positive effect of ASPP module on the obstacle segmentation performance has been studied in our previous work~\cite{bb_iros_2019}.

\begin{figure}
	\centering
      \includegraphics[width=0.6\textwidth]{figures/network_modules.pdf}
      \caption{A detailed visualisation of specific modules used in the proposed network architecture.}
      \label{fig:modules_visualisation}
\end{figure}

\subsection{Architecture modules \cmnt{???}}
\label{subsec:modules}
Our proposed network incorporates three main modules (illustrated in \cref{fig:intro_image} right) to improve the segmentation accuracy and robustness.
\textit{ARM} fuses the visual with inertial information and refines the features of each stage. It
employs global average pooling to capture global context and computes an attention
vector to guide the feature learning.
\textit{FFM} uses batch normalisation to
balance the scales of the features on different levels. By employing the global
average pooling we obtain a weight vector which is used to re-weight the features.
This amount to feature selection and combination.
\textit{ASPP} captures the
global context of the input image at several ranges. %using different receptive fields of different size.



 ------------------ Right camera in the detection experiment for Baselines:
 \begin{comment}
 \\
Right camera &&&&&&\\
\midrule
%\multirow{4}{*}{\STAB{\rotatebox[origin=c]{90}{Right}}}
 U-Net~\cite{ronneberger2015u}           & 18.7                   & 669 [234]    & 4222 [3745] & 47  [32]     & 23.9 [11.0]  & 15.73  \\ 
 PSPNet~\cite{zhao2017pyramid}           & 39.7                   & 350 [107]    & 60   [39]   & 366 [159]    & 62.2 [51.9]  & 17.2        \\ % PSP_2
 DLv2s~\cite{chen2016deeplab}            & 16.5                   & 337 [149]    & 83   [21]   & 379 [117]    & 59.3 [68.3]  & 1.62   \\
 DLv2m~\cite{chen2016deeplab}            & 16.5                   & 267 [121]    & 69   [13]   & 449 [145]    & 50.8 [60.5]  & 1.39   \\ %deeplab2
 \end{comment}
 -----------------------------------------
 
 %A similar result is observed with Modd2 obstacle detection measures in Table~\ref{tab:results_detection}. The water edge is best estimated by Deeplab?, while the number of true positives is maximized by U-Net. However, the high true positive rate comes from a high sensitivity. In contrast to classical measures (Table~\ref{tab:results_segmentation}), Table~\ref{tab:results_detection} reveals that water segmentation is fragmented in U-Net, resulting in extremely large number of false positives, which reduces the F-1 measure. Note that the results are reported for running segmentations separately in left and right images. We observe a consistent performance for all networks. From these results, we selected a single-scale Deeplabv2 architecture for further analysis.

==> related_work_backup.tex <==
Cameras, combined with computer vision algorithms, have proven as a powerful yet affordable obstacle detection devices~\cite{larson2007advances,KristanCYB2015,cane2016saliency,bb_iros_2018,prasad2018overview,muhovivc2019obstacle}. Numerous image-processing methods for obstacle detection have been proposed. In-depth experimental evaluation of background subtraction methods, presented by Prasad~\etal~\cite{prasad2018overview}, has shown that misleading dynamics of water causes a great amount of false-positive detections. Stereo reconstruction methods, such as~\cite{muhovivc2019obstacle} and~\cite{wang2013stereovision}, are only capable of detecting obstacles well above the water surface. Poorly textured and partially submerged objects are likely to be undetected, while the detection of distant obstacles largely depends on the stereo baseline. On the other hand, semantic segmentation methods, based on fitting a structured models to the image~\cite{KristanCYB2015,bb_ras_2018,bb_iros_2018} have achieved promising results and are currently the state-of-the-art on this domain. Segmentation methods are capable of detecting obstacles protruding through the water surface, as well as the floating and distant ones. However, these approaches rely on simple features which fail to correctly address the diversity of a marine scene, thus leading to a poor segmentation in the presence of visual artefacts on water (wakes, sea foam, glitter, environmental reflections, etc.).

Deep convolutional neural networks enable extraction of richer features, mandatory for a good segmentation accuracy in the presence of visual ambiguities. However, a large amount of carefully annotated data is required for training deep neural nets. A large variety of urban datasets have greatly contributed to a rapid development of deep convolutional neural nets~\cite{chen2016deeplab,yu2018bisenet,chen2018encoder,Jeong2018_psp} for autonomous ground vehicles (AGVs) and some of these methods have achieved astonishing semantic segmentation results. But, due to many differences between the AGV and USV domain, these networks cannot be readily applied to the marine environment. For instance, the navigable surface in a maritime domain (water) is non-flat, extremely dynamic and varies significantly in its appearance. Moreover, troubled waters cause USVs to rotate around roll-axis, while ground vehicles do not experience this phenomenon in a typical scenario. 

Although many maritime datasets have been proposed (Modd~\cite{KristanCYB2015}, Modd2~\cite{bb_ras_2018}, IPATCH~\cite{ipatch_dataset}, SEAGULL~\cite{seagull_dataset}, SMD~\cite{smd_prasad2017video}) none of them has a pixel-wise ground truth annotations, required for learning deep segmentation methods. Nonetheless, Lee~\etal~\cite{lee2018image} proposed using a general Faster R-CNN~\cite{ren2015faster} to detect and classify seven different types of ships. Similarly, Yang~\etal~\cite{?} proposed a method for tracking ships in a marine environment, where they have used Faster R-CNN~\cite{ren2015faster} and Yolo3~\cite{?} for ship detection. However, these methods are unable to detect arbitrary obstacles without providing a huge amount of additional training data. Zhan~\etal~\cite{?} proposed a segmentation method for a water component extraction. Their method is composed of VGG-16~\cite{?} backbone in the encoder, followed by a corresponding symmetrical decoder and a CRF~\cite{?} module. The segmentation accuracy continuously improves as online training progresses. However, their method requires a long and non-autonomous ``calibration'' procedure before it starts producing satisfactory results. On the other hand, Cane~\etal~\cite{cane2018evaluating} evaluated three deep semantic segmentation networks (SegNet~\cite{badrinarayanan2017segnet}, ENet~\cite{paszke2016enet}, ESPNet~\cite{mehta2018espnet}) for object detection in maritime surveillance. Fine-tunning was performed on a modified ADE20k dataset, where the original 150 classes were mapped to four custom classes (sea, sky, object and other). Despite the huge amount of images present in ADE20k dataset, only a small subset of 448 images contain visible sea, most of which do not portray a realistic viewpoint of USVs and are detrimental to the learning of deep segmentation methods.

==> rw_backup.tex <==
Yang~\etal~\cite{?} proposed a method for tracking ships in a marine environment. In their work,
they have evaluated two standard deep learning detectors: Faster-RCNN~\cite{?} and Yolo3~\cite{?}. Both detectors
were pretrained on ImageNet~\cite{?} dataset and fine-tuned on a custom dataset consisting of images with six different boat classes:
bulk ship, container ship, warship, passenger ship, speed boat and sailbot.

Scholler~\etal~\cite{?} use long wavelength infrared (LWIR) cameras to detect obstacles in the marine environment. By capturing
and annotating twenty-thousand LWIR images they were able to train three deep learning detectors (FasterRCNN, Yolo and RetinaNet),
which achieve astonishing results on the MS-COCO~\cite{?} and PASCAL VOC~\cite{?}. The selected methods have reached an impressive
mAP result of over 90 percent, however these methods are only able to detect objects seen in the training data and not arbitrary ones.

Zhan~\etal~\cite{?} propose a segmentation method for a water component extraction. Their method uses VGG~\cite{?} backbone as feature
extraction mechanism in the encoder and a symmetrical U-Net like decoder for up-sampling. To further improve the segmentation output,
CRF model is applied at the end of the decoder. Their method was evalu
